Low-Rank Continual Pyramid Vision Transformer: Incrementally Segment Whole-Body Organs in CT with Light-Weighted Adaptation

Deep segmentation networks achieve high performance when trained on specific datasets. However, in clinical practice, it is often desirable that pretrained segmentation models can be dynamically extended to enable segmenting new organs without access to previous training datasets or without training from scratch. This would ensure a much more efficient model development and deployment paradigm accounting for the patient privacy and data storage issues. This clinically preferred process can be viewed as a continual semantic segmentation (CSS) problem. Previous CSS works would either experience catastrophic forgetting or lead to unaffordable memory costs as models expand. In this work, we propose a new continual whole-body organ segmentation model with light-weighted low-rank adaptation (LoRA). We first train and freeze a pyramid vision transformer (PVT) base segmentation model on the initial task, then continually add light-weighted trainable LoRA parameters to the frozen model for each new learning task. Through a holistically exploration of the architecture modification, we identify three most important layers (i.e., patch-embedding, multi-head attention and feed forward layers) that are critical in adapting to the new segmentation tasks, while retaining the majority of the pretrained parameters fixed. Our proposed model continually segments new organs without catastrophic forgetting and meanwhile maintaining a low parameter increasing rate. Continually trained and tested on four datasets covering different body parts of a total of 121 organs, results show that our model achieves high segmentation accuracy, closely reaching the PVT and nnUNet upper bounds, and significantly outperforms other regularization-based CSS methods. When comparing to the leading architecture-based CSS method, our model has a substantial lower parameter increasing rate while achieving comparable performance.

==> problem-formulation.tex <==
Figure \ref{fig:loco_pvt} illustrates the proposed low-rank continual (LoCo) multi-organ segmentation framework. We adopt the UniMISS~\cite{xie2022unimiss} pretrained 3D PVT as backbone. Subsequently, the 3D PVT undergoes further training with the TotalSegmentator dataset~\cite{wasserthal2022totalsegmentator}. After this additional training, the PVT backbone, as depicted by the  blue dashed-line blocks in Figure~\ref{fig:loco_pvt}, is fixed throughout the subsequent training process. For the remaining tasks, let $D = \{D_1,\ldots,D_T\}$ represent the datasets sequence. The model is trained sequentially on each $D_t$ where $t\in\{1,\ldots,T\}$ and will not re-access $D_t$ after training is complete. Consider the $t^{th}$ dataset $D_t = \{X_k^t,Y_k^t\}_{k=1}^{N_t}$ that compromises $O_t$ organ classes, and assuming $(X^t$,$Y^t)$ denote all input images and the corresponding segmentation masks in $D_t$, the prediction map for voxel location $i$ and organ class $c_j$ is given by
\begin{align}
    \hat Y^t(i) = f\left(Y^t(i)=c_j\vert X^t; W_0, W_{L^t}, W_{S^t}\right), 
    \ \ \ 
    \hat{\mathbf Y} = \bigcup_{t=1}^T \hat Y^t ,
    %% formulas must be reviewed, especially how final predictions are performed.
\end{align}
where $f$ denotes the transformer neural networks with frozen parameters $W_0$ trained on initial task and task-specific trainable LoRA parameters $W_{L^t}$ where $L^t = (A_l^t, B_l^t)_{l=1}^{M^t}$ denotes the pairs of low rank matrices for the $t^{th}$ dataset, and $W_{S^t}$ denotes the trainable task-specific Sigmoid output. The final prediction $\hat{\mathbf Y}$ is the union of all previous predictions with possible class overlapping.

==> tabs/css_step.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\small
\centering
\caption{Step-wise mean DSC (\%, $\uparrow$) and forgetting rate (FR) (\%, $\downarrow$) of CSS methods on each dataset and all 121 organs ('All'). EsoTumor is not included since no forgetting rate is calculated for the last continual step. }
\label{tab:supp-step}
\resizebox{1.0\textwidth}{!}{%
\begin{tabular}{>{\raggedright\arraybackslash}p{20mm} *{9}{>{\centering\arraybackslash}p{12mm}}}
\toprule
\multirow{2}{*}{\textbf{Methods}} &
  \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Step}}} &
  \multicolumn{2}{c|}{\textbf{TotalSeg}} &
  \multicolumn{2}{c|}{\textbf{CHO}} &
  \multicolumn{2}{c|}{\textbf{HNO}} &
  \multicolumn{2}{c}{\textbf{All}} \\ \cline{3-10} 
 &
  \multicolumn{1}{c|}{} &
  \textbf{DSC} &
  \multicolumn{1}{c|}{\textbf{FR}} &
  \textbf{DSC} &
  \multicolumn{1}{c|}{\textbf{FR}} &
  \textbf{DSC} &
  \multicolumn{1}{c|}{\textbf{FR}} &
  \textbf{DSC} &
  \textbf{FR} \\ \hline
\multicolumn{10}{c}{\textbf{Order A: TotalSeg $\rightarrow$ CHO $\rightarrow$ HNO $\rightarrow$ EsoTumor}} \\ \hline
\multirow{3}{*}{\textbf{MiB}[1]} &
  \multicolumn{1}{c|}{2} &
  43.07 &
  \multicolumn{1}{c|}{53.15} &
  84.45 &
  \multicolumn{1}{c|}{---} &
  --- &
  \multicolumn{1}{c|}{---} &
  48.63 &
  53.15 \\
 &
  \multicolumn{1}{c|}{3} &
  12.53 &
  \multicolumn{1}{c|}{86.37} &
  39.79 &
  \multicolumn{1}{c|}{52.88} &
  84.62 &
  \multicolumn{1}{c|}{---} &
  21.01 &
  69.63 \\
 &
  \multicolumn{1}{c|}{4} &
  9.18 &
  \multicolumn{1}{c|}{90.01} &
  28.55 &
  \multicolumn{1}{c|}{66.19} &
  9.21 &
  \multicolumn{1}{c|}{89.12} &
  12.19 &
  81.77 \\ \hline
\multirow{3}{*}{\textbf{PLOP}[4]} &
  \multicolumn{1}{c|}{2} &
  58.98 &
  \multicolumn{1}{c|}{35.84} &
  82.66 &
  \multicolumn{1}{c|}{---} &
  --- &
  \multicolumn{1}{c|}{---} &
  62.16 &
  35.84 \\
 &
  \multicolumn{1}{c|}{3} &
  40.11 &
  \multicolumn{1}{c|}{56.37} &
  70.31 &
  \multicolumn{1}{c|}{14.94} &
  82.88 &
  \multicolumn{1}{c|}{---} &
  46.89 &
  35.65 \\
 &
  \multicolumn{1}{c|}{4} &
  37.92 &
  \multicolumn{1}{c|}{58.75} &
  66.98 &
  \multicolumn{1}{c|}{18.97} &
  34.68 &
  \multicolumn{1}{c|}{58.16} &
  41.65 &
  45.29 \\ \hline
\multirow{3}{*}{\textbf{LISMO}[14]} &
  \multicolumn{1}{c|}{2} &
  50.43 &
  \multicolumn{1}{c|}{45.14} &
  84.46 &
  \multicolumn{1}{c|}{---} &
  --- &
  \multicolumn{1}{c|}{---} &
  55.01 &
  45.14 \\
 &
  \multicolumn{1}{c|}{3} &
  15.02 &
  \multicolumn{1}{c|}{83.66} &
  44.24 &
  \multicolumn{1}{c|}{47.62} &
  84.9 &
  \multicolumn{1}{c|}{---} &
  23.59 &
  65.64 \\
 &
  \multicolumn{1}{c|}{4} &
  11.71 &
  \multicolumn{1}{c|}{87.26} &
  43.07 &
  \multicolumn{1}{c|}{49.01} &
  9.22 &
  \multicolumn{1}{c|}{89.14} &
  16.01 &
  75.14 \\ \hline
\multirow{3}{*}{\textbf{SUN}[9]} &
  \multicolumn{1}{c|}{2} &
  91.93 &
  \multicolumn{1}{c|}{0} &
  84.33 &
  \multicolumn{1}{c|}{---} &
  --- &
  \multicolumn{1}{c|}{---} &
  90.91 &
  0 \\
 &
  \multicolumn{1}{c|}{3} &
  91.93 &
  \multicolumn{1}{c|}{0} &
  84.33 &
  \multicolumn{1}{c|}{0} &
  84.79 &
  \multicolumn{1}{c|}{---} &
  90.48 &
  0 \\
 &
  \multicolumn{1}{c|}{4} &
  91.93 &
  \multicolumn{1}{c|}{0} &
  84.33 &
  \multicolumn{1}{c|}{0} &
  84.79 &
  \multicolumn{1}{c|}{0} &
  90.45 &
  0 \\ \hline
\multirow{3}{*}{\textbf{Ours}} &
  \multicolumn{1}{c|}{2} &
  91.07 &
  \multicolumn{1}{c|}{0} &
  81.51 &
  \multicolumn{1}{c|}{---} &
  --- &
  \multicolumn{1}{c|}{---} &
  89.78 &
  0 \\
 &
  \multicolumn{1}{c|}{3} &
  91.07 &
  \multicolumn{1}{c|}{0} &
  81.51 &
  \multicolumn{1}{c|}{0} &
  82.9 &
  \multicolumn{1}{c|}{---} &
  89.30 &
  0 \\
 &
  \multicolumn{1}{c|}{4} &
  91.07 &
  \multicolumn{1}{c|}{0} &
  81.51 &
  \multicolumn{1}{c|}{0} &
  82.9 &
  \multicolumn{1}{c|}{0} &
  89.26 &
  0 \\ \hline
\multicolumn{10}{c}{\textbf{Order B: TotalSeg $\rightarrow$ HNO $\rightarrow$ CHO $\rightarrow$ EsoTumor}} \\ \hline
\multirow{3}{*}{\textbf{MiB}[1]} &
  \multicolumn{1}{c|}{2} &
  23.36 &
  \multicolumn{1}{c|}{74.59} &
  --- &
  \multicolumn{1}{c|}{---} &
  84.87 &
  \multicolumn{1}{c|}{---} &
  31.63 &
  74.59 \\
 &
  \multicolumn{1}{c|}{3} &
  12.08 &
  \multicolumn{1}{c|}{86.86} &
  84.43 &
  \multicolumn{1}{c|}{---} &
  9.88 &
  \multicolumn{1}{c|}{88.36} &
  20.97 &
  86.86 \\
 &
  \multicolumn{1}{c|}{4} &
  11.24 &
  \multicolumn{1}{c|}{87.77} &
  78.65 &
  \multicolumn{1}{c|}{6.85} &
  9.09 &
  \multicolumn{1}{c|}{89.29} &
  20.04 &
  61.30 \\ \hline
\multirow{3}{*}{\textbf{PLOP}[4]} &
  \multicolumn{1}{c|}{2} &
  47.32 &
  \multicolumn{1}{c|}{48.53} &
  --- &
  \multicolumn{1}{c|}{---} &
  83.71 &
  \multicolumn{1}{c|}{---} &
  52.21 &
  48.53 \\
 &
  \multicolumn{1}{c|}{3} &
  32.65 &
  \multicolumn{1}{c|}{64.48} &
  84.15 &
  \multicolumn{1}{c|}{---} &
  25.54 &
  \multicolumn{1}{c|}{69.49} &
  38.59 &
  64.48 \\
 &
  \multicolumn{1}{c|}{4} &
  31.58 &
  \multicolumn{1}{c|}{65.65} &
  79.47 &
  \multicolumn{1}{c|}{5.56} &
  22.78 &
  \multicolumn{1}{c|}{72.79} &
  37.31 &
  48.00 \\ \hline
\multirow{3}{*}{\textbf{LISMO}[14]} &
  \multicolumn{1}{c|}{2} &
  27.21 &
  \multicolumn{1}{c|}{70.40} &
  --- &
  \multicolumn{1}{c|}{---} &
  84.94 &
  \multicolumn{1}{c|}{---} &
  34.97 &
  70.40 \\
 &
  \multicolumn{1}{c|}{3} &
  15.94 &
  \multicolumn{1}{c|}{82.66} &
  84.49 &
  \multicolumn{1}{c|}{---} &
  10.13 &
  \multicolumn{1}{c|}{88.07} &
  24.10 &
  82.66 \\
 &
  \multicolumn{1}{c|}{4} &
  15.01 &
  \multicolumn{1}{c|}{83.67} &
  79.49 &
  \multicolumn{1}{c|}{5.92} &
  8.93 &
  \multicolumn{1}{c|}{89.49} &
  23.14 &
  59.69 \\ \hline
\multirow{3}{*}{\textbf{SUN}[9]} &
  \multicolumn{1}{c|}{2} &
  91.93 &
  \multicolumn{1}{c|}{0} &
  --- &
  \multicolumn{1}{c|}{---} &
  84.79 &
  \multicolumn{1}{c|}{---} &
  90.97 &
  0 \\
 &
  \multicolumn{1}{c|}{3} &
  91.93 &
  \multicolumn{1}{c|}{0} &
  84.33 &
  \multicolumn{1}{c|}{---} &
  84.79 &
  \multicolumn{1}{c|}{0} &
  90.48 &
  0 \\
 &
  \multicolumn{1}{c|}{4} &
  91.93 &
  \multicolumn{1}{c|}{0} &
  84.33 &
  \multicolumn{1}{c|}{0} &
  84.79 &
  \multicolumn{1}{c|}{0} &
  90.45 &
  0 \\ \hline
\multirow{3}{*}{\textbf{Ours}} &
  \multicolumn{1}{c|}{2} &
  91.07 &
  \multicolumn{1}{c|}{0} &
  --- &
  \multicolumn{1}{c|}{---} &
  82.9 &
  \multicolumn{1}{c|}{---} &
  89.97 &
  0 \\
 &
  \multicolumn{1}{c|}{3} &
  91.07 &
  \multicolumn{1}{c|}{0} &
  81.51 &
  \multicolumn{1}{c|}{---} &
  82.9 &
  \multicolumn{1}{c|}{0} &
  89.30 &
  0 \\
 &
  \multicolumn{1}{c|}{4} &
  91.07 &
  \multicolumn{1}{c|}{0} &
  81.51 &
  \multicolumn{1}{c|}{0} &
  82.9 &
  \multicolumn{1}{c|}{0} &
  89.26 &
  0 \\ 
  \bottomrule
\end{tabular}
}
\end{table}
